Playing Games with your PET: Extending the Partial Exploration Tool to Stochastic Games

We present version 2.0 of the Partial Exploration Tool (PET), a tool for verification of probabilistic systems. We extend the previous version by adding support for stochastic games, based on a recent unified framework for sound value iteration algorithms. Thereby, PET2 is the first tool implementing a sound and efficient approach for solving stochastic games with objectives of the type reachability/safety and mean payoff. We complement this approach by developing and implementing a partial-exploration based variant for all three objectives. Our experimental evaluation shows that PET2 offers the most efficient partial-exploration based algorithm and is the most viable tool on SGs, even outperforming unsound tools.

==> 0_space.tex <==
% == FLOATS ==
%
\setlength{\textfloatsep}{0.5\textfloatsep} % Space below/above a float if its [t]
\setlength{\intextsep}{0.5\intextsep} % Space below/above a float if its [h]
\setlength{\floatsep}{0.5\floatsep} % Space between floats
\setlength{\abovecaptionskip}{0.5\abovecaptionskip}
\setlength{\belowcaptionskip}{0.5\belowcaptionskip}

\setcounter{topnumber}{2}
\setcounter{totalnumber}{3}
\renewcommand{\topfraction}{0.8}

% == EQUATIONS ==
% done inside document

% == FOOTNOTES ==

\setlength{\footnotesep}{0.25cm}
\setlength{\skip\footins}{0.5cm}

% == NAUGHTY BITS ==

%\renewcommand{\baselinestretch}{0.97} % >=0.97
\advance\textwidth4mm % <= 6mm
\advance\hoffset-2mm
%\advance\textheight3mm
%\advance\voffset-1.5mm
%
%\setlength{\marginparwidth}{3.3cm}
%\setlength{\marginparsep}{0.1cm}

%\let\subparagraph\relax
%\usepackage{titlesec}
%\titlespacing{\section}{0pt}{2ex}{1ex}
%\titlespacing{\subsection}{0pt}{1ex}{0.5ex}
%\titlespacing{\subsubsection}{0pt}{0.5ex}{0.25ex}
%\titlespacing{\paragraph}{0pt}{0.5ex}{1ex}


%\setdefaultleftmargin{1.5em}{1.5em}{}{}{}{}



